Soft Augmentation for Image Classification

Modern neural networks are over-parameterized and thus rely on strong regularization such as data augmentation and weight decay to reduce overfitting and improve generalization. The dominant form of data augmentation applies invariant transforms, where the learning target of a sample is invariant to the transform applied to that sample. We draw inspiration from human visual classification studies and propose generalizing augmentation with invariant transforms to soft augmentation where the learning target softens non-linearly as a function of the degree of the transform applied to the sample: e.g., more aggressive image crop augmentations produce less confident learning targets. We demonstrate that soft targets allow for more aggressive data augmentation, offer more robust performance boosts, work with other augmentation policies, and interestingly, produce better calibrated models (since they are trained to be less confident on aggressively cropped/occluded examples). Combined with existing aggressive augmentation strategies, soft target 1) doubles the top-1 accuracy boost across Cifar-10, Cifar-100, ImageNet-1K, and ImageNet-V2, 2) improves model occlusion performance by up to $4\times$, and 3) halves the expected calibration error (ECE). Finally, we show that soft augmentation generalizes to self-supervised classification tasks. Code available at https://github.com/youngleox/soft_augmentation

==> figures/calibration.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/images/calibration_wideresnet28d0_2_cifar100.pdf}
    \caption{Soft Augmentation + TrivialAugment (SA+TA) improves model confidence calibration and mean confidence level. Left:  SA+TA reduces expected calibration error (ECE, in legend) by more than half by mitigating both over-confidence in the high model confidence region and under-confidence in the low model confidence region. Right: SA+TA reduces the number of unconfident predictions and increase mean prediction confidence from $83.37\%$ to $86.64\%$. All results are 3 runs of WideResNet-28 on Cifar-100. Shaded area and error bars indicate standard error of the mean.}
    \label{fig:calibration}
\end{figure}

==> figures/curves.tex <==
\begin{figure}[h]
    \vspace{-4mm}
    \centering
    \begin{tabular}{c c}
        \includegraphics[width=0.4\linewidth]{cvpr2023-author_kit-v1_1-1/figures/Tang et al. fig1f.png}
        \includegraphics[width=0.4\linewidth]{cvpr2023-author_kit-v1_1-1/figures/soft_curves.pdf}
    \end{tabular}
    
    \caption{Left: human classification performance under various occlusion levels from Figure 1F of Tang \etal~\cite{tang2018recurrent}. Right: power functions used in Soft Augmentation.}
    \label{fig:curves}
    \vspace{-3mm}
\end{figure}

==> figures/ece.tex <==
\begin{table}[h]
    \vspace{-3mm}
    \centering
    
        \caption{Soft Augmentation improves calibration of ResNet-50 on ImageNet. }
        \vspace{-3mm}

    \begin{tabular}{c c c c c}
        \toprule
         Dataset & \multicolumn{4}{c}{ECE} \\
           & Baseline & RA & SA & RA+SA \\
        \midrule
         ImageNet-1K & 5.11 & 4.09 & 3.17 & 2.78 \\

         ImageNet-V2 & 9.91 & 8.84 & 3.24 & 3.18 \\
        \bottomrule
    \end{tabular}
    \label{tab:ece}
    \vspace{-2mm}
\end{table}

==> figures/mixup2.tex <==
\begin{figure}[h]
    \vspace{-4mm}
    \centering
    \begin{tabular}{c c}
        \includegraphics[width=0.55\linewidth]{cvpr2023-author_kit-v1_1-1/figures/mixup.png}
        \includegraphics[width=0.28\linewidth]{cvpr2023-author_kit-v1_1-1/figures/sa.png}
    \end{tabular}
    
    \caption{Left and Center: effect of Mixup from Zhang \etal~\cite{tang2018recurrent}. Right: Soft Augmentation can be considered as a generalized version of Mixup}
    \label{fig:mixup}
    \vspace{-3mm}
\end{figure}

==> figures/robustness.tex <==
\begin{table*}[h]
    \centering
        \caption{Soft Augmentation improves occlusion robustness of ResNet-18 on Cifar-100. $32 \times 32$ validation images of Cifar-100 are cropped with offsets $t_x, t_y$ randomly drawn from $U(-\lambda, \lambda)$. $\lambda$ is set to $\{0,8,16,24,32\}$ to create a range of mean occlusion levels. Both RandAugment (RA) and Soft Augmentation (SA) improve occlusion robustness independently. The combined performance improvements are larger than the sum of the individual ones ($\Delta_{SA+RA} > \Delta_{RA} + \Delta_{SA}$).}
    \resizebox{0.7\textwidth}{!}{
    \begin{tabular}{c c c c c c}
        \toprule
         ResNet-18 &  \multicolumn{5}{c}{Cifar-100 Top-1 Error} \\
         \midrule
         Occlusion Level ($\lambda$)  & 0 & 8 & 16 & 24 & 32 \\
         \midrule
         Baseline  
         & $20.80_{\pm 0.11} $ 
         & $ 24.57_{\pm 0.13} $ 
         & $ 43.83_{\pm 0.39} $ 
         & $ 68.41_{\pm 0.21} $
         & $ 81.89_{\pm 0.15} $\\
         
         RA
         & $20.99_{\pm 0.11} $ 
         & $ 23.37_{\pm 0.07} $ 
         & $ 36.60_{\pm 0.16} $ 
         & $ 61.02_{\pm 0.09} $
         & $ 77.13_{\pm 0.19} $\\
         
         ($\Delta_{RA}$)
         & (+0.19)
         & (-1.20)
         & (-7.23)
         & (-7.39)
         & (-4.76) \\
         
         SA
         & $18.31_{\pm 0.17}$ 
         & $ 23.93_{\pm 0.11} $ 
         & $ 42.13_{\pm 0.52} $ 
         & $ 64.83_{\pm 0.56} $
         & $ 79.52_{\pm 0.33} $\\
         
         ($\Delta_{SA}$)
         & (-2.49)
         & (-0.64)
         & (-1.70)
         & (-3.58)
         & (-2.37) \\
         
         SA + RA 
         & $\bm{18.10_{\pm 0.20}}$ 
         & $\bm{20.73_{\pm 0.10}}$ 
         & $\bm{31.08_{\pm 0.16}}$ 
         & $\bm{52.98_{\pm 0.85}}$
         & $\bm{72.18_{\pm 0.28}}$ \\
         
         ($\Delta_{SA+RA}$)
         & (-2.70)
         & (-3.84)
         & (-12.75)
         & (-15.43)
         & (-9.71) \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:robustness}
\end{table*}

\begin{comment}
\begin{table*}[h]
    \centering
        \caption{Comparing SA with other methods. Top-1 errors of ResNet-18 on Cifar-100 are reported.}
    \begin{tabular}{c c c c c c c}
        \toprule
         ResNet-18 &  Cifar-100-C & \multicolumn{5}{c}{Cifar-100 Crop} \\
         \midrule
          &  & 0 & 8 & 16 & 24 & 32 \\
         Baseline  & $ 50.09{\pm 0.07} $ & \\
         RA  & $ 43.20{\pm 0.20} $ & \\
         SA  & $ 51.59{\pm 0.15}$ & \\
         SA + RA & $\bm{42.10_{\pm 0.15}}$ & \\
        \bottomrule
    \end{tabular}

    \label{tab:robustness}
\end{table*}
\end{comment}

==> figures/robustness_imagenet.tex <==
\begin{table*}[h]
    \centering
        \caption{Soft Augmentation improves occlusion robustness of ResNet-50 on ImageNet. $224 \times 224$ validation images of ImageNet are occluded with randomly placed square patches that cover $\lambda$ of the image area. $\lambda$ is set to $\{0\%,20\%,40\%,60\%,80\% \}$ to create a range of occlusion levels. Both RandAugment (RA) and Soft Augmentation (SA) improve occlusion robustness independently. Combining RA with SA reduces Top-1 error by up to 17\%. At 80\% occlusion level, SA+RA achieves more than $\bm{4\times}$ \textbf{accuracy improvement} over baseline (18.98\% vs 3.42\%).}
    \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{c c c c c c}
        \toprule
         ResNet-50 &  \multicolumn{5}{c}{ImageNet Top-1 Accuracy} \\
         \midrule
         Occlusion Level ($\lambda$)  & 0\% & 20\% & 40\% & 60\% & 80\% \\
         \midrule
         Baseline  
         & $ 77.38_{\pm <0.01} $ 
         & $ 64.48_{\pm 0.15} $ 
         & $ 42.78_{\pm 0.20} $ 
         & $ 19.14_{\pm 0.64} $
         & $ 3.42_{\pm 0.40} $\\
         
         RA*
         & $ 77.98_{\pm 0.00} $ 
         & $ 66.70_{\pm 0.00} $ 
         & $ 47.30_{\pm 0.00} $ 
         & $ 24.83_{\pm 0.00} $
         & $ 6.41_{\pm 0.00} $\\
         
         ($\Delta_{RA}$)
         & (+0.59)
         & (+2.22)
         & (+4.51)
         & (+5.69)
         & (+2.99) \\
         
         SA
         & \underline{$ 78.33_{\pm 0.02}$ }
         & \underline{$ 68.80_{\pm 0.09} $ }
         & \underline{$ 52.82_{\pm 0.13} $ }
         & \underline{$ 34.87_{\pm 0.09} $ }
         & \underline{$ 17.15_{\pm 0.16} $ } \\
         
         ($\Delta_{SA}$)
         & (+0.95)
         & (+4.32)
         & (+10.04)
         & (+15.73)
         & (+13.73) \\
         
         SA + RA 
         & $\bm{78.73_{\pm 0.05}}$ 
         & $\bm{69.88_{\pm 0.05}}$ 
         & $\bm{54.06_{\pm 0.10}}$ 
         & $\bm{36.65_{\pm 0.05}}$
         & $\bm{18.98_{\pm 0.12}}$ \\
         
         ($\Delta_{SA+RA}$)
         & (+1.35)
         & (+5.40)
         & (+11.28)
         & (+17.51)
         & (+15.56) \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:robustness_imagenet}
\end{table*}

\begin{comment}
\begin{table*}[h]
    \centering
        \caption{Comparing SA with other methods. Top-1 errors of ResNet-18 on Cifar-100 are reported.}
    \begin{tabular}{c c c c c c c}
        \toprule
         ResNet-18 &  Cifar-100-C & \multicolumn{5}{c}{Cifar-100 Crop} \\
         \midrule
          &  & 0 & 8 & 16 & 24 & 32 \\
         Baseline  & $ 50.09{\pm 0.07} $ & \\
         RA  & $ 43.20{\pm 0.20} $ & \\
         SA  & $ 51.59{\pm 0.15}$ & \\
         SA + RA & $\bm{42.10_{\pm 0.15}}$ & \\
        \bottomrule
    \end{tabular}

    \label{tab:robustness}
\end{table*}
\end{comment}

==> section/98_checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
\begin{comment}


The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\end{comment}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec:discussion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{There is no particular risk associated with this research beyond increasing the accuracy of machine learning models. However, improving the calibration of machine learning models more reliable and trustworthy.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Example Python implementation of the soft crop augmentation and the loss function are included in Section\ref{sec:implementation}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Details are included in Sections \ref{sec:exp} and \ref{sec:appendix_exp}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report standard error of the mean of three independent runs for all experiments.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section \ref{sec:appendix_exp}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{Licensing details are described in \ref{sec:appendix_exp}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We include Python implementation examples of Soft Augmentation in \ref{sec:implementation}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All datasets and models used are publicly available.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{We use the standard Cifar-10/100, ImageNet-1K, and ImageNet-V2 datasets. While ImageNet does contain people, it is generally believed to have no offensive content, and it is arguably one of the most widely used datasets in computer vision.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

